Compression Forcing: Hierarchical History Tokenization Enables Flexible World Models

Effective world modeling requires compressing salient history information that facilitates future prediction. However, most existing approaches inherit tokenization and conditioning mechanisms from video generation, where objectives are centered around perceptual realism rather than predictive utility. This discrepancy limits the world model's effectiveness, especially in environments dominated by visual nuisances or task-irrelevant background details. To this end, we introduce Compression Forcing (CF), a general framework that aligns history compression with the predictive objective of world modeling. Compression Forcing features Dynamics-Aware Tokenization (DAT), a novel tokenization method that compresses history observations into a sequence ordered by decreasing dynamics saliency. Built on a diffusion backbone, this structure enables Hierarchical History Guidance (HG-H), allowing selective amplification of dynamics-salient information during inference. Extensive experiments across various environments demonstrate improved prediction fidelity, physical realism, and downstream decision-making performance, establishing Compression Forcing as a highly flexible and effective approach for world modeling.

==> preamble/arxiv_title.tex <==
\makeatletter
    \renewcommand{\abstractname}{\normalsize Abstract}
    \makeatother
    
    \makeatletter
    \renewcommand{\maketitle}{
    \newpage
    \null
    %\vskip 2em
    \begingroup
    \raggedright
    %\let\footnote\@gobble
    {\LARGE \bfseries \@title \par}
    \vskip 1.5em
    {\large
    \lineskip .5em
    \begin{tabular}[t]{l}
    \@author
    \end{tabular}\par}
    \vskip 1em
    {\large \@date \par}
    \endgroup
    \par
    %\vskip 1.5em
}
\makeatother


% Metadata commands (inspired by fairmeta.cls)
\makeatletter
% Helper command to add items to a list
\newcommand\addtometadatalist[5][]{%
  \begingroup
  \if\relax#3\relax\def\sep{}\else\def\sep{#5}\fi
  \let\protect\@unexpandable@protect
  \xdef#3{\expandafter{#3}\sep #4[#1]{#2}}%
  \endgroup
}

% Metadata list and format
\newcommand\metadatalist{}
\newcommand\metadataformat[2][]{{\small \textbf{#1:} #2}}
\newcommand\metadata[2][]{\addtometadatalist[#1]{#2}{\metadatalist}{\metadataformat}{\\}}
\makeatother

% Convenience commands for common metadata
\newcommand{\paperwebsite}[1]{\metadata[Website]{\url{#1}}}
\newcommand{\papercode}[1]{\metadata[Code]{\url{#1}}}
\newcommand{\paperdocs}[1]{\metadata[Documentation]{\url{#1}}}
\newcommand{\paperblog}[1]{\metadata[Blog]{\url{#1}}}
\newcommand{\paperdate}[1]{\metadata[Date]{#1}}
